Improving Engagement and Efficacy of mHealth Micro-Interventions for Stress Coping: an In-The-Wild Study

Sustaining long-term user engagement with mobile health (mHealth) interventions while preserving their high efficacy remains an ongoing challenge in real-world well-being applications. To address this issue, we introduce a new algorithm, the Personalized, Context-Aware Recommender (PCAR), for intervention selection and evaluate its performance in a field experiment. In a four-week, in-the-wild experiment involving 29 parents of young children, we delivered personalized stress-reducing micro-interventions through a mobile chatbot. We assessed their impact on stress reduction using momentary stress level ecological momentary assessments (EMAs) before and after each intervention. Our findings demonstrate the superiority of PCAR intervention selection in enhancing the engagement and efficacy of mHealth micro-interventions to stress coping compared to random intervention selection and a control group that did not receive any intervention. Furthermore, we show that even brief, one-minute interventions can significantly reduce perceived stress levels (p=0.001). We observe that individuals are most receptive to one-minute interventions during transitional periods between activities, such as transitioning from afternoon activities to bedtime routines. Our study contributes to the literature by introducing a personalized context-aware intervention selection algorithm that improves engagement and efficacy of mHealth interventions, identifying key timing for stress interventions, and offering insights into mechanisms to improve stress coping.

==> 5-discussion.tex <==
% we should consider the following structure to align with the methods 

% \subsection{Effectiveness of Timing and Content (Aligned with Aim1)}
% % Discuss the implications of the findings on what aspects of the timing and content were most effective and why.

% \subsection{Implications of Short-Term Stress Reduction (Aligned with Aim2)}
% % Discuss the broader implications of the short-term stress reduction observed in the study.

% \subsection{Personalization and Long-Term Benefits (Aligned with Aim3)}
% % Discuss the potential for long-term integration of personalized stress-coping strategies into daily life, based on the study's findings.

\section{Discussion}
\label{section:Discussion}

In this four-week study utilizing a 2x2 factorial design, we investigated the timing of engagement with stress-reducing micro-interventions across various stress stages among  \( N = 27 \) parents of young children. We also examined the influence of personalized, context-aware content. Employing three delivery conditions—Control (no interventions), Random interventions, and personalized interventions via the \pcar model—and four categories of intervention content, we found that participants predominantly engaged with interventions during transitional periods of their day. These periods notably included transitions from work to afternoon activities with their children and from these activities to bedtime routines.

.






\subsection{User Engagement}
In \ref{finding: user engagement }, a clear trend of declining user engagement was observed over the course of the experiment, as evidenced in Figure \ref{fig: engagement_patient}. This decline could be attributed to users becoming disengaged or losing interest in the intervention. It is plausible that the limited data contributed to this trend, and a more comprehensive and extended study could provide further insights into this issue. The observed decline in user engagement underscores the importance of sustaining user interest and engagement in real-time stress intervention studies.

Conversely, the high variability witnessed during the study in the acceptance rate of our participants suggests that a larger dataset is needed to draw definitive conclusions. Moreover, this variability underscores the importance of considering individual differences in user behavior when designing and implementing real-time stress intervention systems. It also highlights the need for adaptive approaches that can tailor interventions to the unique preferences and needs of each user, ensuring that the interventions are relevant and engaging for all participants. Addressing this variability is crucial for enhancing the effectiveness of stress interventions and improving user satisfaction and adherence, particularly in the context of human-computer interaction studies.

\subsection{The association between personality traits and acceptance rates}
%this section should discuss the implications of the big five results

\subsection{Effect of Digital Micro-Interventions}
%TODO: Add to this part more discussion related to results shown in the findings
In ~\ref{finding: Impact of Personalization }, we found that digital micro-interventions were effective in mitigating momentary stress levels when the timing of the intervention was determined by the ~\ref{subsubsection: Just-A-Minute Component} and the content was randomly selected for the users. We utilized delta stress measurements as a key metric for evaluating the efficacy of various interventions. 


\subsection{Momentary vs Relative Stress Levels}
In our analysis in ~\ref{finding: stress_reward_time}, it's evident that participants exhibited varied stress levels on a day-to-day basis. While the average stress levels provided insightful feedback from each participant's perspective, the concept of 'reward', defined as the difference between subsequent stress levels, offered a more generalized way to understand the impact of stress interventions.

Notably, the variance in stress levels before and after intervention was considerably high, suggesting that individual responses to interventions were diverse. In contrast, the variance in the 'reward' or the change in stress levels was more consistent among participants. This discrepancy in variance underscores the complexity of stress responses and the multifaceted nature of factors influencing them. While the broader range in stress levels indicates a wide spectrum of individual experiences throughout the day, the narrower range in 'reward' suggests that the relative change in stress, post-intervention, tends to be more meaningful for learning across participants. This observation prompts further exploration into the underlying mechanisms and factors that contribute to these patterns, potentially guiding more tailored intervention strategies for our personalized intervention recommender.

\subsection{Impact of Personalization}
Although existing literature suggests that personalized interventions enhance both engagement and outcomes in stress management ~\cite{nahum2018just}, and that repetitive content can lead to a boredom effect ~\cite{paredes2014poptherapy}, our study did not find a significant difference in stress reduction between the personalized and random recommendation groups. This discrepancy could be due to several factors. First, the system may have lacked sufficient data or time to fully understand the participants' behaviors and preferences.


Another consideration pertains to the study design. To minimize user disturbance, we opted not to explicitly collect feedback on the intervention experience. Instead, we implicitly gathered this information through delta stress measurements (reward). This approach may have limited our ability to accurately assess user preferences, as perceived stress could be influenced by external factors unrelated to the specific exercises.










==> pseudocode_sarsa.tex <==




\begin{algorithm}
    \caption{Accelerated SARSA-LFA for Contextual Environments: Learn function \text{\( Q: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R} \)}}
    \label{alg:accelerated-sarsa-lfa}
    \begin{algorithmic}[1]
        \Procedure{AcceleratedSARSA-LFA}{$\mathcal{S}$, A, R, T, $\alpha, \gamma, \lambda$}

            \State Initialize weight vector \( w \in \mathbb{R}^d \) arbitrarily
            \State Initialize \( e: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R} \) with 0.
            \While{True}
                \State Observe current state \( s \) and context \( \mathcal{C} \)
                \State Select action \( a \) based on \( \pi(s) \)
                \State \( r \gets R(s, a) \)
                \State \( s' \gets T(s, a) \)
                \State \( a' \gets \pi(s') \)
                \State \( e(s, a) \gets e(s, a) + 1 \)
                \State \( \delta \gets r + \gamma \cdot Q(s', a') - Q(s, a) \)
                \State Update all weights \( w_i \)
                \State \( e(s, a) \gets \gamma \cdot \lambda \cdot e(s, a) \)
                \If{Accelerated}
                    \For{each \( g \) s.t \( g_{a} = s_{a} \)}
                        \State \( g' \gets T(g, a) \)
                        \State \( a_g' \gets \pi(g') \)
                        \State \( \delta \gets r + \gamma \cdot Q(g', a_g') - Q(g,a) \)
                        \State \( Q(g, a) \gets Q(g, a) + \alpha\cdot \delta \)
                    \EndFor
                \EndIf
                \State \( s \gets s' \)
                \State \( a \gets a' \)
            \EndWhile
        \EndProcedure
    \end{algorithmic}
\end{algorithm}



